Multiscale Memory Comparator Transformer for Few-Shot Video Segmentation

Few-shot video segmentation is the task of delineating a specific novel class in a query video using few labelled support images. Typical approaches compare support and query features while limiting comparisons to a single feature layer and thereby ignore potentially valuable information. We present a meta-learned Multiscale Memory Comparator (MMC) for few-shot video segmentation that combines information across scales within a transformer decoder. Typical multiscale transformer decoders for segmentation tasks learn a compressed representation, their queries, through information exchange across scales. Unlike previous work, we instead preserve the detailed feature maps during across scale information exchange via a multiscale memory transformer decoding to reduce confusion between the background and novel class. Integral to the approach, we investigate multiple forms of information exchange across scales in different tasks and provide insights with empirical evidence on which to use in each task. The overall comparisons among query and support features benefit from both rich semantics and precise localization. We demonstrate our approach primarily on few-shot video object segmentation and an adapted version on the fully supervised counterpart. In all cases, our approach outperforms the baseline and yields state-of-the-art performance. Our code is publicly available at https://github.com/MSiam/MMC-MultiscaleMemory.

==> core/background.tex <==
\label{sec:bg}
We start with covering the necessary background for multiscale multigrid methods in classical approaches before deep learning to motivate why multigrid indicates a bidirectional information flow. Multigrid methods~\cite{briggs2000multigrid,brandt1977multi} were mainly used to solve huge systems of partial differential equations (PDEs) in a computationally efficient manner and with reduced residual error. An iterative approach that tries to approximate the solution is computed on a discretized finite dimensional approximation space. The discretization process may result in a too fine grid that consequently entails solving large system of equations without considering smoothness constraints that can help alleviate errors. Thus, the proposition of multigrid methods is to operate on multiple levels of discretization allowing for interactions among fine and coarse grid when deriving the approximate solution. Consider the system of equations that needs to be solved as, $Au=f$, where $u$ is the exact solution and we approximate it with, $v$, and $A$ represents our system of equations. The algebraic error in this case is, $e = u - v$, and the residual error of our approximate solution can be computed as, $r = f - Av$. If re-arranging the residual equation we end up with, $Av= f - r$, and since we know that $Au=f$, we can write the relationship between the residual and error as $Ae=r$. In multigrid methods~\cite{briggs2000multigrid} the solution is first discretized on multiple levels of resolution. For simplicity we initially consider only two levels of discretization with corresponding grids $\Omega^{h}, \Omega^{2h}$. The coarser grid, $\Omega^{2h}$, will have better convergence rate and can aid in decreasing the residual error instead of using only the fine grid, $\Omega^{h}$. We will use the superscript $\textbf{\_}^h$ to denote the version used in the corresponding discretized grid $\Omega^h$ and similarly for other reoslution levels. The operators that can transfer from grid $\Omega^h$ to $\Omega^{2h}$ is, $I_h^{2h}$ through interpolation. The known correction scheme in a multigrid approach, which is called V-cycle~\cite{briggs2000multigrid}, uses the following recursive solution:\\
 
\begin{algorithm}
    \begin{algorithmic}[1]
    \Statex \texttt{$v^h \leftarrow \text{VCycle}^h(v^h, f^h)$}
    \State \texttt{Relax $\eta_1$ times on $A^hu^h=f^h$ with an initial guess $v^h$}
    \If{$\Omega^h$ is the coarsest grid}
        \State \texttt{go to 10}.
    \Else
        \State \texttt{$r^{2h} \leftarrow I^{2h}_h (f^h - A^hv^h)$}
        \State \texttt{$e^{2h} \leftarrow 0$}
        \State \texttt{$e^{2h} \leftarrow \text{VCycle}^{2h}(e^{2h}, r^{2h})$ }
    \EndIf
    \State \texttt{Correct $v^h \leftarrow v^h + I^{h}_{2h}e^{2h}$}
    \State \texttt{Relax $\eta_2$ times on $A^hu^h=f^h$ with initial guess $v^h$}
    \end{algorithmic} 
    \caption{V-Cycle correction scheme in a multigrid manner.}
    \label{alg:tti}
\end{algorithm}

It can be clearly seen that this recursive solution allows for a bidirectional information flow between the different resolution levels to ensure smooth solutions with lower error.

==> core/intro_old.tex <==
Few-shot learning is concerned with investigating the generalization ability of models beyond the closed set of training classes to novel unseen classes guided by a few labelled examples. The few labelled examples (\ie the support set) are used as a guide to classify or segment target images (\ie the query set). Few-shot learning approaches can be categorized into~\cite{chen2019closer}: (i) metric learning methods~\cite{qi2018low,snell2017prototypical} (\ie learning to compare), (ii) hallucination based methods~\cite{wang2018low} (\ie learning to augment) and (iii) initialization based methods~\cite{finn2017model} (\ie learning to fine-tune). In metric learning methods the focus is on learning a comparator between the support set and query set, where the embeddings of the same class should be closer together and further apart from other classes. It has been widely adopted in different few-shot tasks such as, few-shot classification~\cite{chen2019closer,qi2018low}, few-shot segmentation~\cite{min2021hypercorrelation,wang2019panet} and few-shot video object segmentation~\cite{chen2021delving}. 

Few-shot video object segmentation, where the query set to be segmented is a video, is a crucial task that can help reduce the annotation cost required to label large-scale video datasets. It can serve a variety of applications in autonomous systems~\cite{cen2021deep} and medical image processing~\cite{ross2020robust} which require the model to learn from few labelled examples for novel classes that are beyond the closed set of training classes with abundant labels. It can also help bridge the gap between developing and developed countries, where the former lacks the resources necessary to annotate large-scale labelled datasets that are required in a variety of tasks that serves the community such as, the use of satellite imagery in agricultural monitoring and crop management~\cite{segarra2020remote}.

\textbf{Related research.} Metric learning (\ie learning to compare) is a widely adopted approach in fewshot segmentation~\cite{wang2019panet,siam2019amp,siam2020weakly}, video object segmentation~\cite{chen2021delving} and video understanding~\cite{yang2021few}. However, there are still limitations in the current techniques available. It is important to consider multiple levels of resolution (\ie coarse, mid and fine resolution) and feature abstraction (\ie features extracted from early, mid and late stages) when designing the support-to-query comparator, which is currently lacking in few-shot video object segmentation and understanding. Although, in few-shot segmentation multiscale processing on correlation tensors between the support and query sets has been considered~\cite{min2021hypercorrelation}, the model can be confused by erroneous correlations especially at the finest resolution. In our work we investigate meta-learning a multiscale transformer with learnable keys that can better separate the background from the novel class while allowing bidirectional information flow across scales in a multigrid manner. 

Incorporating multiscale processing in transformers is an emerging topic within the context of different tasks such as action recognition~\cite{fan2021multiscale,li2021improved} and panoptic segmentation~\cite{cheng2021masked}. However, it was either explored solely on the encoder side~\cite{fan2021multiscale,li2021improved,wang2022crossformer} which is not sufficient when computing dense predictions, or the transformer decoder~\cite{cheng2021masked} design led to a loss of the spatiotemporal dimension during the multiscale processing. On the other hand, in our approach it is crucial to preserve the spatiotemporal dimension in the multiscale processing without losing important details required for the final segmentation in order to enable our proposed multiscale multigrid approach. Additionally we rather operate on correlation tensors rather than features maps unlike previous works. Close to our work is the task of finding dense correspondences robust to different variations where a recent method that captures global dependencies from dense feature matches using transformers has been proposed~\cite{cho2021cats}. Nonetheless, our work explores meta-learning a transformer decoder with learnable keys that can better separate background from the novel class, with the downstream task of few-shot video segmentation and understanding. Additionally, our multiscale multigrid comparator allows for bidirectional information flow across scales which makes it even more suitable for the target fewshot task and to the best of our knowledge has not been explored earlier within transformers.

{\bf Contributions.} In this paper we investigate multiscale processing within the few-shot video object segmentation task. We propose to meta-learn a multiscale multigrid transformer comparator that operates on correlation tensors from different resolution levels and learns a set of keys to separate the novel class from the background in a multigrid formulation. We look into the different forms of information flow between the different levels of resolution similar to classical multigrid methods~\cite{briggs2000multigrid} which allow for bidirectional information flow. We show that bidirectional information flow similar to multigrid methods outperforms simple coarse-to-fine processing. Our multigrid multiscale approach can better avoid erroneous correlations that usually exist at the finest resolution level. Overall, our contributions are threefold. (i) We propose a multiscale multigrid transformer decoder that operates on correlation tensors between the support and query set features on multiple levels of resolution. Key to our multiscale transformer decoder is allowing bidirectional information flow between coarse-to-fine and early-to-late stage feature. (ii) Another key enabler to the previous multigrid multiscale transformer decoder is that we preserve the spatiotemporal dimension in the multiscale processing, unlike other methods that squeezes the spatiotemporal dimension~\cite{cheng2021masked}. We rather learn to combine the different learned keys per pixel and time frame within the spatiotemporal grid. (iii) We present the first attempt to meta-learn a multi-scale comparator between the support and query sets for the few-shot video segmentation task and show case the versatility of our approach through extending it to few-shot video understanding where actor/action classes are segmented. 
%(iv) in our extension to the few-shot actor/action segmentation we propose to meta-learn a multiscale static/dynamic comparator that uses correlation tensors which represent both the static (\ie information delivered from a single frame such as texture) and dynamic (\ie information delivered from consecutive set of frames such as motion) factors.

%We show the generality of our approach on different tasks: (i) fewshot video segmentation and (ii) few-shot common action localisation which goes one further step beyond actor segmentation and rather predicts the action as well.



%earning visual correspondences has generally been heavily in previous studies~\cite{} where the downstream task was mainly keypoint matching.
%Recently, outside of few-shot learning literature and tailored towards the general task of visual correspondance a transformer based approach that captures global dependancies from correlation tensors has been investigated.  
